Compression of descriptor models for mobile applications

Deep neural networks have demonstrated state-of-the-art performance for feature-based image matching through the advent of new large and diverse datasets. However, there has been little work on evaluating the computational cost, model size, and matching accuracy tradeoffs for these models. This paper explicitly addresses these practical metrics by considering the state-of-the-art HardNet model. We observe a significant redundancy in the learned weights, which we exploit through the use of depthwise separable layers and an efficient Tucker decomposition. We demonstrate that a combination of these methods is very effective, but still sacrifices the top-end accuracy. To resolve this, we propose the Convolution-Depthwise-Pointwise(CDP) layer, which provides a means of interpolating between the standard and depthwise separable convolutions. With this proposed layer, we can achieve an 8 times reduction in the number of parameters on the HardNet model, 13 times reduction in the computational complexity, while sacrificing less than 1% on the overall accuracy across theHPatchesbenchmarks. To further demonstrate the generalisation of this approach, we apply it to the state-of-the-art SuperPoint model, where we can significantly reduce the number of parameters and floating-point operations, with minimal degradation in the matching accuracy.

==> figures/hardnet++_4way_decomposition.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Rank},
        ylabel={mAP [\%]},
        xmin=0, xmax=8,
        xtick={0, 1, 2, 3, 4, 5, 6, 7, 8},
        %ytick={0.0, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1},
        ymin=0, ymax=20,
        grid style=dashed
    ]
 
    %% Matching
    \addplot[color=blue, mark=square]
    coordinates {
    %(1, 2.33716e-05)(2, 0.00022924)(3, 0.000786942)(4, 0.00335734)(5,0.00616695)(6, 0.0130343)(7,  0.0162087)(8, 0.0167435)
    (1, 2.33716e-03)(2, 0.022924)(3, 0.0786942)(4, 0.335734)(5,0.616695)(6, 1.30343)(7,  1.62087)(8, 1.67435)
    
    %(0, 0.55385) % R
    };
    
    %% Retrieval (average over all noises)
    \addplot[color=green, mark=square]
    coordinates {
    %(1, 0.033451501)(2, 0.062409351)(3, 0.072942839)(4, 0.106352529)(5,0.115942229)(6, 0.140147771)(7, 0.144758843)(8, 0.153647429)
    (1, 3.3451501)(2, 6.2409351)(3, 7.2942839)(4, 10.6352529)(5, 11.5942229)(6, 14.0147771)(7, 14.4758843)(8, 15.3647429)
    
    %(0, 0.744902) % R
    };
    
    \legend{Image Matching, Patch Retrieval}
    
    %\node [above] at (axis cs:  1, 3.3451501) {$32h$};
    
    \end{axis}
    \begin{axis}[
        xlabel={Number of parameters},
        xtick = {0, 1077, 2154, 3231, 4308, 5385, 6462, 7539, 8616},
        xmin = 0, xmax = 8616,
        ymin = 0, ymax = 20,
        tick label style={font=\tiny},
        axis y line=none,
        axis x line*=top,
        xlabel near ticks,
        xmajorgrids=true
    ]
    \end{axis}
    
\end{tikzpicture}
\caption{HardNet++ task performance using weight rank decomposition. The weights for each layer are decomposed across each of the 4 dimensions. }
\label{table:hardnet_tensor_decomposition_performance}
\end{figure}

==> figures/hardnet++_parameters_per_layer.tex <==
\begin{figure}[H]
\centering
\begin{tikzpicture}
    \begin{axis}[
        ybar,
        enlargelimits=0.15,
        ylabel={\# Parameters},
        ytick=\empty,
        xlabel={Layer \#},
        xtick = {1, 2, 3, 4, 5, 6, 7},
        nodes near coords,
        nodes near coords align={vertical},
        every node near coord/.style={font=\tiny},
        ]
    \addplot coordinates {(1, 288) (2, 9216) (3, 18432) (4, 36864) (5, 73728) (6, 147456) (7, 1048576)};
    \end{axis}
\end{tikzpicture}
\caption{Number of weights used for each convolutional layer (ignoring the bias)}
\label{fig:hardnet_layer_parameter_count}
\end{figure}

==> figures/l2net_complexity.tex <==
\begin{figure*}[ht]
\centering
% ----- COMPLEXITY ---- %
%\scalebox{1.0}[0.5]{%
\resizebox{!}{0.2\textheight}{%
\begin{tikzpicture}
    \begin{axis}[
        width  = 0.85*\textwidth,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        bar width=7pt,
        ymajorgrids = true,
        xlabel = {(a)   Layer},
        ylabel = {Computational cost (MFLOPs)},
        xlabel style={font=\Large},
        ylabel style={font=\Large},
        symbolic x coords={1,2,3,4,5,6,7},
        xtick = data,
        scaled y ticks = false,
        enlarge x limits=0.25,
        ymin=0,
        legend cell align=left,
        legend style={
                font=\large,
                at={(0.95,0.8)},
                anchor=south east,
                column sep=1ex
        }
    ]
        \addplot[style={bblue,fill=bblue,mark=none}]
            coordinates {
                (1, 0.29)
                (2, 9.44)
                (3, 4.72)
                (4, 9.44)
                (5, 1.18)
                (6, 9.44)
                (7, 1.05)
            };

        \addplot[style={rred,fill=rred,mark=none}]
             coordinates {
                (1, 0.04)
                (2, 1.34)
                (3, 0.60)
                (4, 1.20)
                (5, 0.14)
                (6, 1.12)
                (7, 0.02)
             };

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {
                (2, 3.48)
                (3, 1.87)
                (4, 1.39)
                (5, 0.49)
                (6, 1.64)
                (7, 0.14)
             };

        \legend{Original, DepthSep, Tucker}
    \end{axis}
\end{tikzpicture}
}%
% ----- PARAMS ---- %
\resizebox{!}{0.2\textheight}{%
\begin{tikzpicture}
    \begin{axis}[
        width  = 0.85*\textwidth,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        bar width=7pt,
        ymajorgrids = true,
        xlabel = {(b)   Layer},
        ylabel = {Parameters},
        xlabel style={font=\Large},
        ylabel style={font=\Large},
        symbolic x coords={1,2,3,4,5,6,7},
        xtick = data,
        scaled y ticks = false,
        enlarge x limits=0.25,
        ymin=0, ymax=1200000, ymode=log,
        legend cell align=left,
        legend style={
                font=\large,
                at={(0.3,0.8)},
                anchor=south east,
                column sep=1ex
        }
    ]
    \addplot[style={bblue,fill=bblue,mark=none}]
      coordinates{
        (1, 288)
        (2, 9216)
        (3, 18432)
        (4, 36864)
        (5, 73728)
        (6, 147456)
        (7, 1048576)
    };
    
    \addplot[style={rred,fill=rred,mark=none}]
      coordinates{
        (1, 41)
        (2, 1312)
        (3, 2336)
        (4, 4672)
        (5, 8768)
        (6, 17536)
        (7, 24576)
    };
    
    \addplot[style={ggreen,fill=ggreen,mark=none}]
      coordinates{
        (2, 3396)
        (3, 3288)
        (4, 5446)
        (5, 13587)
        (6, 25589)
        (7, 143168)
    };
    \legend{Original, DepthSep, Tucker}
    \end{axis}
    \end{tikzpicture}
}%
\caption{Complexity of the L2Net architecture. Left (a) shows the number of floating point operations in each layer for standard convolutions, depthwise separable layers, and the Tucker decomposition. Right  (b) presents the number of parameters on a logarithmic axis.}
\label{fig:l2net_params_complexity}
\end{figure*}

==> figures/mse_pw_weights.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Rank},
        ylabel={Reconstruction error (MSE)},
        xmin=1, xmax=10,
        grid style=dashed,
        cycle list name=exotic list,
        legend style={at={(rel axis cs:0.9,0.35)}, above left, name=legend, draw=none},
        /pgf/number format/precision=5
    ]
 
    % Layer 2
    \addplot
    coordinates {
    (1, 0.009378009475767612) (2, 0.008270095102488995) (3, 0.00720784068107605) (4, 0.006203739903867245) (5, 0.005325453355908394) (6, 0.004544951021671295) (7, 0.0039025424048304558) (8, 0.003272256813943386) (9, 0.002749094972386956) (10, 0.002260859590023756)
    };
    
    % Layer 3
    \addplot
    coordinates {
    (1, 0.0038160430267453194) (2, 0.0035114260390400887) (3, 0.0032263710163533688) (4, 0.002956218784675002) (5,  0.0027118874713778496) (6, 0.0024915682151913643) (7, 0.0022758226841688156) (8, 0.0020700348541140556) (9, 0.001869824482128024) (10, 0.0016808084910735488)
    };
    
    % Layer 4
    \addplot
    coordinates {
    (1, 0.004502058494836092) (2, 0.004164304584264755) (3, 0.003855776507407427) (4, 0.0035669920034706593) (5, 0.0032979799434542656) (6, 0.003041542135179043) (7, 0.0028016550932079554) (8, 0.002578306943178177) (9, 0.0023932678159326315) (10, 0.002212901832535863)
    };
    
    % Layer 5
    \addplot
    coordinates {
    (1, 0.0019837631843984127) (2, 0.0018631953280419111) (3, 0.0017498693196102977) (4, 0.001650733407586813) (5, 0.0015626589301973581) (6,  0.0014815239701420069) (7,  0.0014095966471359134) (8, 0.0013439081376418471) (9, 0.0012857314432039857) (10, 0.0012307330034673214)
    };

    % Layer 6
    \addplot
    coordinates {
    (1, 0.001987352967262268) (2, 0.001900460571050644) (3, 0.0018214730080217123) (4, 0.001745291636325419) (5, 0.0016695756930857897) (6, 0.001597731257788837) (7, 0.0015273562166839838) (8, 0.001459072926081717) (9, 0.00139232212677598) (10, 0.0013298268895596266)
    };
    
    % Layer 7
    \addplot
    coordinates {
    (1, 0.0016411114484071732) (2, 0.0016056380700320005) (3, 0.001571230823174119) (4, 0.0015379935503005981) (5, 0.0015062196180224419) (6, 0.0014745229855179787) (7, 0.0014432952739298344) (8, 0.0014122123830020428) (9,  0.001382110407575965) (10, 0.0013524023815989494) 
    };
    
    %\addlegendentry[yshift=10pt]{\textbf{Layer \#}}
    \addlegendentry{2}
    \addlegendentry{3}
    \addlegendentry{4}
    \addlegendentry{5}
    \addlegendentry{6}
    \addlegendentry{7}

    \end{axis}
    
    \node [above, font=\bfseries] (legendtitle) at (legend.north) {Layer \#};
    \node [fit=(legendtitle)(legend), draw, inner sep=0pt] {};
\end{tikzpicture}

==> figures/total_error_pw_weights.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Rank},
        ylabel={Total reconstruction error},
        xmin=1, xmax=10,
        grid style=dashed,
        cycle list name=exotic list,
        %legend style={at={(rel axis cs:1.25,0.35)}, above left, name=legend, draw=none}
    ]
 
    % Layer 2
    \addplot
    coordinates {
    (1, 9.603082
) (2, 8.468577385
) (3, 7.380828857
) (4, 6.352629662
) (5, 5.453264236
) (6, 4.654029846
) (7, 3.996203423
) (8, 3.350790977
) (9, 2.815073252
) (10, 2.31512022
)
    };
    
    % Layer 3
    \addplot
    coordinates {
    (1, 15.63051224
) (2, 14.38280106
) (3, 13.21521568
) (4, 12.10867214
) (5, 11.10789108
) (6, 10.20546341
) (7, 9.321769714
) (8, 8.478862762
) (9, 7.658801079
) (10, 6.884591579
)
    };
    
    % Layer 4
    \addplot
    coordinates {
    (1, 18.44043159
) (2, 17.05699158
) (3, 15.79326057
) (4, 14.61039925
) (5, 13.50852585
) (6, 12.45815659
) (7, 11.47557926
) (8, 10.56074524
) (9, 9.802824974
) (10, 9.064045906
)
    };
    
    % Layer 5
    \addplot
    coordinates {
    (1, 32.50197601
) (2, 30.52659225
) (3, 28.66985893
) (4, 27.04561615
) (5, 25.60260391
) (6, 24.27328873
) (7, 23.09483147
) (8, 22.01859093
) (9, 21.06542397
) (10, 20.16432953
)
    };

    % Layer 6
    \addplot
    coordinates {
    (1, 32.56079102
) (2, 31.137146
) (3, 29.84301376
) (4, 28.59485817
) (5, 27.35432816
) (6, 26.17722893
) (7, 25.02420425
) (8, 23.90545082
) (9, 22.81180573
) (10, 21.78788376
)
    };
    
    % Layer 7
    \addplot
    coordinates {
    (1, 26.88796997
) (2, 26.30677414
) (3, 25.74304581
) (4, 25.19848633
) (5, 24.67790222
) (6, 24.15858459
) (7, 23.64694977
) (8, 23.13768768
) (9, 22.64449692
) (10, 22.15776062
) 
    };
    
    %\addlegendentry{2}
    %\addlegendentry{3}
    %\addlegendentry{4}
    %\addlegendentry{5}
    %\addlegendentry{6}
    %\addlegendentry{7}

    \end{axis}
    
    %\node [above, font=\bfseries] (legendtitle) at (legend.north) {Layer \#};
    %\node [fit=(legendtitle)(legend), draw, inner sep=0pt] {};
    
\end{tikzpicture}

==> tables/superpoint.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{0.4\linewidth}{!}{%
    \begin{tabular}{|c|c|c|c|}
    
        \hline
        \textbf{Model} & \textbf{Illumination changes}
        & \textbf{Viewpoint changes} \\
        \hline
        FAST & 57.6 & 41.5 \\
        \hline
        Harris & 63.0 & 48.1 \\
        \hline
    
    \end{tabular}%
    }
    \medbreak
    \resizebox{0.85\linewidth}{!}{%
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        %\multicolumn{14}{c}{} \\
        
        \hline
        \multicolumn{9}{|c|}{\textbf{Layer offsets}} & \multicolumn{1}{c|}{\textbf{Illumination changes}} & \multicolumn{1}{c|}{\textbf{Viewpoint changes}} & \multicolumn{1}{c|}{\textbf{Compression ratio}} & \multicolumn{2}{c|}{\textbf{Operations (GFLOPs)}} \\
        \hline
        % VGG
        \multicolumn{1}{|c}{\textbf{\#2}} & \multicolumn{1}{c}{\textbf{\#3}} & \multicolumn{1}{c}{\textbf{\#4}} & \multicolumn{1}{c}{\textbf{\#5}} & \multicolumn{1}{c}{\textbf{\#6}} & \multicolumn{1}{c}{\textbf{\#7}} & 
        \multicolumn{1}{c|}{\textbf{\#8}} & 
        % Head
        \multicolumn{1}{|c}{\textbf{\#9}} &
        \multicolumn{1}{c|}{\textbf{\#10}} &
        % Empty cols
        \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Backbone} & \multicolumn{1}{c|}{Head} \\
        
        % Data
        \hline
        % 942083
        \multicolumn{9}{|c|}{\textit{Original}} & \multicolumn{1}{c|}{67.3} & % 0.6729
        \multicolumn{1}{c|}{39.5} & % 0.3954
        \multicolumn{1}{c|}{$1\times$} &
        \multicolumn{1}{c|}{5.81} & \multicolumn{1}{c|}{0.37} \\
        \hline
        
        % 293875
        \multicolumn{1}{|c}{2} & \multicolumn{1}{c}{2} & 
        \multicolumn{1}{c}{2} & \multicolumn{1}{c}{2} &
        \multicolumn{1}{c}{2} & \multicolumn{1}{c}{2} &
        \multicolumn{1}{c}{2} & \multicolumn{1}{|c}{2} &
        \multicolumn{1}{c|}{2} &
        \multicolumn{1}{c|}{67.0} & % 0.6702
        \multicolumn{1}{c|}{38.8} & % 0.3882
        \multicolumn{1}{c|}{$\bm{3.21\times}$} &
        \multicolumn{1}{c|}{\textbf{1.61}} & \multicolumn{1}{c|}{\textbf{0.15}} \\
        
        % 316696
        \multicolumn{1}{|c}{5} & \multicolumn{1}{c}{5} & 
        \multicolumn{1}{c}{5} & \multicolumn{1}{c}{5} &
        \multicolumn{1}{c}{5} & \multicolumn{1}{c}{5} &
        \multicolumn{1}{c}{5} & \multicolumn{1}{|c}{5} &
        \multicolumn{1}{c|}{5} &
        \multicolumn{1}{c|}{\textbf{67.3}} & % 0.6732
        \multicolumn{1}{c|}{\textbf{40.5}} & % 0.4052
        
        % Below are wrong results with 3x3 conv instead of 1x1 (mistake)
        %\multicolumn{1}{c|}{0.6731} & 
        %\multicolumn{1}{c|}{0.3944} & 
        \multicolumn{1}{c|}{$2.97\times$}  &
        \multicolumn{1}{c|}{1.83} & \multicolumn{1}{c|}{0.16} \\
        
        \hline
        % 365019
        \multicolumn{1}{|c}{2} & \multicolumn{1}{c}{4} & 
        \multicolumn{1}{c}{4} & \multicolumn{1}{c}{8} &
        \multicolumn{1}{c}{8} & \multicolumn{1}{c}{16} &
        \multicolumn{1}{c}{16} & \multicolumn{1}{|c}{16} &
        \multicolumn{1}{c|}{16} &
        \multicolumn{1}{c|}{66.8} & 
        \multicolumn{1}{c|}{39.6} & 
        \multicolumn{1}{c|}{$2.58\times$}  &
        \multicolumn{1}{c|}{1.74} & \multicolumn{1}{c|}{0.18} \\
        \hline
        
    \end{tabular}%
    }
    %, with the non-maxima suppression set to 4.
    \caption{Repeatability for the classical detectors and the SuperPoint variants on the \textit{HPatches} dataset. All the models are evaluated on 1000 interest points. The first 8 layers correspond to the shared VGG net architecture, whereas the last 2 layers form  the detector head. The FLOP calculation assumes an input image of size $240 \times 320 \times 3$.}
    \label{table:superpoint_detector_cdp_layer}
\end{table*}
